OpenVVC: a Lightweight Software Decoder for the Versatile Video Coding Standard

In the recent years, users requirements for higher resolution, coupled with the apparition of new multimedia applications, have created the need for a new video coding standard. The new generation video coding standard, called Versatile Video Coding (VVC), has been developed by the Joint Video Experts Team, and offers coding capability beyond the previous generation High Efficiency Video Coding (HEVC) standard. Due to the incorporation of more advanced and complex tools, the decoding complexity of VVC standard compared to HEVC has approximately doubled. This complexity increase raises new research challenges to achieve live software decoding. In this context, we developed OpenVVC, an open-source software decoder that supports a broad range of VVC functionalities. This paper presents the OpenVVC software architecture, its parallelism strategy as well as a detailed set of experimental results. By combining extensive data level parallelism with frame level parallelism, OpenVVC achieves real-time decoding of UHD video content. Moreover, the memory required by OpenVVC is remarkably low, which presents a great advantage for its integration on embedded platforms with low memory resources. The code of the OpenVVC decoder is publicly available at https://github.com/OpenVVC/OpenVVC

==> openVVC_2020 2/Glossary.tex <==
% A
\newacronym{avc}{AVC}{Advanced Video Coding}
\newacronym{ai}{AI}{All Intra}
\newacronym{alf}{ALF}{Adaptive Loop Filter}
\newacronym{aom}{AOM}{Alliance for Open Media}
\newacronym{amvp}{AMVP}{Advanced Motion Vector Prediction}
\newacronym{avx}{AVX}{Advanced Vector eXtensions}

% B
\newacronym{bt}{BT}{Binary Tree}
\newacronym{bh}{BTH}{Binary Tree Horizontal}
\newacronym{bv}{BTV}{Binary Tree Vertical}
\newacronym{bdr}{BD-BR}{Bj\o ntegaard Delta BitRate}
\newacronym{bdpsnr}{BD-PSNR}{Bj\o ntegaard Delta PSNR}
\newacronym{bdof}{BDOF}{Bi-Directional Optical Flow}

% C
\newacronym{ctu}{CTU}{Coding Tree Unit}
\newacronym{cu}{CU}{Coding Unit}
\newacronym{cnn}{CNN}{Convolution Neural Network}
\newacronym{ctc}{CTC}{Common Test Conditions}
\newacronym{crc}{CRC}{Complexity Reduction Configuration}
\newacronym{cpu}{CPU}{Central Processing Unit}
\newacronym{cabac}{CABAC}{Context Adaptive Binary Arithmetic Coding}
\newacronym{CTC}{CTC}{Common Test Conditions}
\newacronym{ccitt}{CCITT}{International Telegraph and Telephone Consultative Committee}
\newacronym{cb}{CB}{Coding Block}
\newacronym{ciip}{CIIP}{Combined Intra/Inter Prediction}
\newacronym{cc-alf}{CC-ALF}{Cross Component ALF}
\newacronym{cclm}{CCLM}{Cross Component Linear Model}

% D
\newacronym{dl}{DL}{Deep Learning}
\newacronym{DCT}{DCT}{Discrete Cosine Transform}
\newacronym{DST}{DST}{Discrete Sine Transform}
\newacronym{dmvr}{DMVR}{Decoder-side Motion Vector Refinement}
\newacronym{dpb}{DPB}{Decoded Picture Buffer}
\newacronym{dbf}{DBF}{Deblocking Filter}

% E
\newacronym{ecore}{E-core}{Efficient core}

% F
\newacronym{fhd}{FHD}{Full High Definition}
\newacronym{fps}{fps}{Frames Per Second}

%G
\newacronym{gop}{GOP}{Group of Pictures}
\newacronym{gpu}{GPU}{Graphical Processing Unit}
\newacronym{gpm}{GPM}{Geometric Partitioning Mode}

\newacronym{gpp}{GPP}{General Purpose Processor}



% H
\newacronym{hevc}{HEVC}{High Efficiency Video Coding}
\newacronym{hdr}{HDR}{High Dynamic Range}
\newacronym{hi}{HI}{Horizontal Inconsistency}
\newacronym{isp}{ISP}{Intra Sub-Partitionning}
\newacronym{hm}{HM}{HEVC Model}
\newacronym{hd}{HD}{High Definition}
\newacronym{HFR}{HFR}{High Frame Rate}
\newacronym{hvs}{HVS}{Human Visual System}

%I
\newacronym{iso}{ISO}{International Organization for Standardization}
\newacronym{iec}{IEC}{International Electrotechnical Commission}
\newacronym{itu}{ITU}{International Telecommunication Union}
\newacronym{ict}{ICT}{Inter-Component Transform}

%J
\newacronym{jvet}{JVET}{Joint Video Experts Team}
\newacronym{jem}{JEM}{Joint Exploration Model}

% Q
\newacronym{qt}{QT}{Quad Tree}
\newacronym{qp}{QP}{Quantization Parameter}
\newacronym{qtbt}{QTBT}{Quad Tree Binary Tree}

%L
\newacronym{lmcs}{LMCS}{Luma Mapping with Chroma Scaling}
\newacronym{ld}{LD}{Low-Delay}
\newacronym{ldp}{LDP}{Low-Delay P}
\newacronym{ldb}{LDB}{Low-Delay B}
\newacronym{lfnst}{LFNST}{Low-Frequency Non-Separable Transform}

% M
\newacronym{mpm}{MPM}{Most Probable Mode}
\newacronym{mv}{MV}{Motion Vector}
\newacronym{ml}{ML}{Machine Learning}
\newacronym{mi}{MI}{Mutual Information}
\newacronym{mdf}{MDF}{Motion Divergence Field}
\newacronym{mc}{MC}{Motion Compensation}
\newacronym{me}{ME}{Motion Estimation}
\newacronym{mpeg}{MPEG}{Moving Picture Experts Group}
\newacronym{mtt}{MTT}{Multi-Type Tree}
\newacronym{MOS}{MOS}{Mean Opinion Score}
\newacronym{MTS}{MTS}{Multiple Transform Selection}
\newacronym{mip}{MIP}{Matrix-based Intra Prediction}
\newacronym{mimd}{MIMD}{Multiple Instructions on Multiple Data}
\newacronym{mse}{MSE}{Mean Squared Error}
\newacronym{mrl}{MRL}{Multiple Reference Line}

% P
\newacronym{pcore}{P-core}{Performance core}
\newacronym{pdf}{Pdf}{Probability Density Function}
\newacronym{pu}{PU}{Prediction Unit}
\newacronym{psnr}{PSNR}{Peak Signal to Noise Ratio}
\newacronym{pmd}{PMD}{Pyramid Motion Divergence}
\newacronym{poc}{POC}{Picture Order Count}
\newacronym{pps}{PPS}{Picture Parameter Set}
\newacronym{prof}{PROF}{Prediction Refinement with Optical Flow}
% R
\newacronym{rd}{RD}{Rate Distorsion}
\newacronym{rdo}{RDO}{Rate Distorsion Optimization}
\newacronym{ra}{RA}{Random Access}
\newacronym{rgb}{RGB}{Red Blue Green}
\newacronym{rf}{RF}{Random Forest}
\newacronym{rs}{RS}{Rectangular Slice}


%S
\newacronym{satd}{SATD}{Sum of Absolute Transform Differences}
\newacronym{svm}{SVM}{Support Vector Machines}
\newacronym{si}{SI}{Spatial Information}
\newacronym{scc}{SCC}{Screen Coding Content}
\newacronym{simd}{SIMD}{Single Instruction on Multiple Data}
\newacronym{shvc}{SHVC}{Scalable High Efficiency Video Coding}
\newacronym{sao}{SAO}{Sample Adaptive Offset}
\newacronym{SPS}{SPS}{Sequence Parameter Set}
\newacronym{sisd}{SISD}{Single Instruction on Single Data}
\newacronym{ssim}{SSIM}{Structural SIMilarity}
\newacronym{sbtmvp}{SbTMVP}{Subblock-based Temporal Motion Vector Prediction}
\newacronym{samviq}{SAMVIQ}{Subjective Assessment Methodology for Video Quality}
\newacronym{sse}{SSE}{Streaming SIMD Extensions}
\newacronym{sota}{SOTA}{State-of-the-Art}

% T
\newacronym{tu}{TU}{Transform Unit}
\newacronym{ti}{TI}{Temporal Information}
\newacronym{tt}{TT}{Ternary Tree}
\newacronym{tth}{TTH}{Ternary Tree Horizontal}
\newacronym{ttv}{TTV}{Ternary Tree Vertical}
\newacronym{trs}{TRS}{Tile and Rectangular Slice}
\newacronym{tl}{TL}{Temporal Layer}
\newacronym{tmvp}{TMVP}{Temporal Motion Vector Prediction}

% U
\newacronym{uhd}{UHD}{Ultra High Definition}

% V
\newacronym{vvc}{VVC}{Versatile Video Coding}
\newacronym{vi}{VI}{Vertical Inconsistency}
\newacronym{vceg}{VCEG}{Video Coding Experts Group}
\newacronym{vtm}{VTM}{VVC Test Model}
\newacronym{vmaf}{VMAF}{Video Multi-Method Assessment Fusion}

% W
\newacronym{wpp}{WPP}{Wavefront Parallel Processing}
\newacronym{waip}{WAIP}{Wide Angular Intra Prediction}

